NeuS2: Fast Learning of Neural Implicit Surfaces for Multi-view Reconstruction

Recent methods for neural surface representation and rendering, for example NeuS, have demonstrated the remarkably high-quality reconstruction of static scenes. However, the training of NeuS takes an extremely long time (8 hours), which makes it almost impossible to apply them to dynamic scenes with thousands of frames. We propose a fast neural surface reconstruction approach, called NeuS2, which achieves two orders of magnitude improvement in terms of acceleration without compromising reconstruction quality. To accelerate the training process, we parameterize a neural surface representation by multi-resolution hash encodings and present a novel lightweight calculation of second-order derivatives tailored to our networks to leverage CUDA parallelism, achieving a factor two speed up. To further stabilize and expedite training, a progressive learning strategy is proposed to optimize multi-resolution hash encodings from coarse to fine. We extend our method for fast training of dynamic scenes, with a proposed incremental training strategy and a novel global transformation prediction component, which allow our method to handle challenging long sequences with large movements and deformations. Our experiments on various datasets demonstrate that NeuS2 significantly outperforms the state-of-the-arts in both surface reconstruction accuracy and training speed for both static and dynamic scenes. The code is available at our website: https://vcai.mpi-inf.mpg.de/projects/NeuS2/ .

==> Sec/OLD_2_Related_Work.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Related work} \label{sec:related}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par
%

\subsection{Static scene reconstruction.} 
%

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Classical MVS
%
\par 
%
\textbf{Multi-view stereo.} Traditional multi-view 3D reconstruction has been explored for decades, which can be categorized into depth-based and voxel-based methods. Depth-based methods reconstruct a point cloud by identifying point correspondences across images and applying triangulation. These methods are often post-processed by Poisson surface reconstruction to form surfaces. The reconstruction quality is heavily affected by the accuracy of correspondence matching, and the difficulties in finding reliable correspondences for objects without rich texture and non-Lambertian surfaces lead to incomplete and noisy 3D reconstruction. Voxel-based methods side-step the difficulties in explicit correspondence matching by recovering occupancy and color in a voxel grid from multi-view images with a photometric consistency criterion. However, the reconstruction results of these methods are limited to low resolution due to the high memory consumption of voxel grids. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Learning-based 
%
\par 
%
\textbf{Neural Implicit Representations for Multi-view Reconstruction.} Recent neural implicit representations have shown  
%
\MH{Todo}
\cite{wang2021neus}
\cite{idr_yariv2020multiview}
\cite{muller2022instant_ngp}
\cite{saito2019pifu}
\cite{Oechsle2021}
\cite{yariv2021volume}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par 
%
\textbf{Dynamic scene reconstruction.}
%
Next, we review works that focus on dynamic scene reconstruction.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Shape from template
%
\par 
%
\textit{Shape from template.}
%
\MH{Todo}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% NRSFM
%
\par 
%
\textit{Non-rigid structure from motion.}
%
\MH{Todo}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Shape-from-x
%
\par 
%
\textit{Shape-from-x.}
%
\MH{Todo}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Learning-based
%
\par 
%
\textit{Learning-based methods.}
%
\MH{Todo}
%
\cite{pumarola2021d_nerf}
\cite{Tretschk2021_NonRigid}
\cite{xian2020spacetime}
\cite{park2020nerfies}
\cite{pumarola2020dnerf}
\cite{yang2021lasr}

==> Sec/OLD_2_Related_Work_new.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Related Work} \label{sec:related}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Multi-view Stereo.} Traditional multi-view 3D reconstruction has been explored for decades, which can be categorized into depth-based and voxel-based methods. Depth-based methods~\cite{barnes2009patchmatch,furukawa2009accurate,galliani2016gipuma, schonberger2016pixelwise} reconstruct a point cloud by identifying point correspondences across images and applying triangulation. 
% These methods are often post-processed by Poisson surface reconstruction to form surfaces. 
The reconstruction quality is heavily affected by the accuracy of correspondence matching, and the difficulties in finding reliable correspondences for objects without rich texture and non-Lambertian surfaces lead to incomplete and noisy 3D reconstruction. 
Voxel-based methods~\cite{de1999poxels,broadhurst2001probabilistic, seitz1999photorealistic} side-step the difficulties in explicit correspondence matching by recovering occupancy and color in a voxel grid from multi-view images with a photometric consistency criterion. However, the reconstruction of these methods is limited to low resolution due to the high memory consumption of voxel grids. 
%




\textbf{Classical multi-view 4D Reconstruction.} 
A large body of work in multi-view 4D reconstruction is to utilize a precomputed deformable model and deform the model to fit the silhouette and/or the dense pixel color of the multi-view images. These methods~\cite{carranza2023,Vlasic2008,Ahmed2008,Aguiar2008,Xu2018,Habermann2019} are broadly used in human performance capture. However, they require a high-quality deformable model, and struggle with fine details recovery and topology change handeling. 
Different from these works, our method abandons the need for a precomputed model, can reconstruct detailed results and handle topology changes. 
The most relevant to our work is \cite{Collet2015}, which is also a model-free method.  \cite{Collet2015} first combines RGB stereo, IR stereo, and Shape from Silhouette to reconstruct high-quality point clouds for each frame, and then employs Poisson surface reconstruction~\cite{Kazhdan2006} to obtain meshes; next, it selects keyframes and tracks them over sequences of frames to produce temporally coherent subsequences. 
While \cite{Collet2015} can produce impressive results, it requires both RGB and depth as input and the whole pipeline consists of many sophisticated and time-consuming procedures. 
In this paper, we only focus on how to efficiently get high-quality reconstruction per frame and leave the mesh tracking over sequences out of the scope of this paper. 
Different from \cite{Collet2015}, we only needs RGB as input and can learn the high-quality geometry and appearance for each frame in an end-to-end manner in 20 seconds per frame. 

\textbf{Neural Implicit Representations.} Neural implicit representations have made remarkable achievements in novel view synthesis~\cite{sitzmann2019scene,lombardi2019neural,kaza2019differentiable,mildenhall2020nerf,liu2020neural, sitzmann2019deepvoxels} and 3D/4D reconstruction~\cite{saito2019pifu,saito2020pifuhd,yariv2020multiview,niemeyer2020differentiable,kellnhofer2021neural,jiang2020sdfdiff,liu2020dist,Oechsle2021ICCV,wang2021neus,yariv2021volume}. NeRF~\cite{mildenhall2020nerf} models 3D geometry as a density field and appearance as a radiance field, which are represented by MLPs, and then applies a volume rendering technique to learn the fields from multi-view RGB images. Though it has shown high-quality results in the novel view synthesis task, it cannot extract high-quality surfaces since the density field used lacks surface constraints. Some works~\cite{yariv2020multiview,niemeyer2020differentiable,jiang2020sdfdiff,liu2020dist,Oechsle2021ICCV,wang2021neus,yariv2021volume} thus propose to use surface representation, such as Signed Distance Function (SDF) and occupancy field. A representative work among them, NeuS~\cite{wang2021neus}, combines SDF with an unbiased volume rendering method for high-quality surface reconstruction. However, the training of NeuS is very slow, requiring over 8 hours for one scene, and NeuS only works on static scene reconstruction. Instead, our method significantly accelerates the training of NeuS from 8 hours to about \yiming{40 seconds}, and the training can be further accelerated to 20 seconds per frame when applied to dynamic scene reconstruction. 

Another line of related work is the follow-up works of NeRF~\cite{mildenhall2020nerf}. Some methods~\cite{mvsnerf,grf2020,yu2020pixelnerf,wang2021ibrnet,liu2022neuray} reduce training cost by pretraining NeRF on various scenes to obtain generalizable features. Other works~\cite{yu_and_fridovichkeil2021plenoxels,SunSC22,muller2022instant_ngp} introduce voxel-grid features to represent 3D properties for fast training. However, these methods cannot extract high-quality surfaces as they inherit the volume density field as the geometry representation from NeRF~\cite{mildenhall2020nerf}. Instead, our method can achieve high-quality surface reconstruction as well as fast training. 
% For example, InstantNGP~\cite{muller2022instant_ngp} presents an efficient encoding of 3D position, called multi-resolution hash encoding, and provides a CUDA implementation to accelerate the NeRF training. However, applying these techniques to learn neural implicit surfaces is not trivial, which will be elaborated later in Sec. xxx. We thus present an efficient calculation of the second-order derivatives of MLPs to enable CUDA acceleration in training, and a progressive training strategy for more stable training and faster convergence. 
For dynamic scene modeling, many works~\cite{tretschk2020nonrigid,park2020nerfies, pumarola2020dnerf,park2021hypernerf,Li2020NeuralSF,xian2020spacetime} propose to disentangle a 4D scene into a shared canonical space and a deformable field per frame. While these works make the training for dynamic scenes more efficient, the training is still time-consuming,  taking more than 2 days to train one sequence with 200 frames. Furthermore, these methods are not able to handle large movements and reconstruct high-quality surfaces. Some works in human performance modeling~\cite{su2021anerf,liu2021neural,peng2021animatable,chen2021animatable,xu2021hnerf,2021narf,zhang2021stnerf,peng2020neural,kwon2021neural,Gao2022neuralnovelactor} can model large movements by introducing a deformable template as a prior. 
Instead, our method can handle large movements, does not require a deformable template and thus is not restricted to a specific dynamic object. Moreover, we can learn high-quality surfaces of dynamic scenes for about 20 seconds per frame. 

\textbf{Concurrent Work.}
\cite{tineuvox} represents a 4D scene with a time-aware voxel feature, where a multi-distance interpolation is proposed and applied to model small and large motions. \cite{liu2022devrf} proposes a static-to-dynamic learning paradigm, which first learns a neural voxel field for one frame and then jointly trains a deformation field for the rest of the frames. These two  methods focus on the novel view synthesis task and thus are not designed to reconstruct high-quality surfaces, which is different from our goal of achieving high-quality surface geometry and appearance models. Also the two methods train for many frames together, while our method proposes an incremental training strategy. 
Voxurf~\cite{Voxurf} proposes a voxel-based surface representation for multi-view 3D reconstruction, and designs a two-stage training strategy, a dual color network and a hierarchical geometry feature to improve the results.  While it enables 20x speedup over the baselines (i.e., NeuS~\cite{wang2021neus}), our proposed method is over 3x faster than Voxurf and achieves better geometry quality when compared with Voxurf's results reported in the paper. Also, Voxurf is not designed for dynamic scene reconstruction. 
~\cite{zhao2022human} proposes a method for human modeling and rendering. It first reconstructs a neural surface representation for each frame; then it applies non-rigid deformation to obtain a temporally coherent mesh sequence, which is similar to the mesh tracking process in ~\cite{Collet2015}. Our work focuses on the first part, that is,  fast reconstruction of dynamic scenes, where we exploit the temporal consistency between two consecutive frames to accelerate the learning of dynamic representation. Therefore, our work is orthogonal to ~\cite{Collet2015}, and can be integrated into ~\cite{zhao2022human} as the first step. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par 
%

% \textbf{Dynamic scene reconstruction.}
% %
% Next, we review works that focus on dynamic scene reconstruction.
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % Shape from template
% %
% \par 
% %
% \textit{Shape from template.}
% %
% \MH{Todo}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % NRSFM
% %
% \par 
% %
% \textit{Non-rigid structure from motion.}
% %
% \MH{Todo}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % Shape-from-x
% %
% \par 
% %
% \textit{Shape-from-x.}
% %
% \MH{Todo}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % Learning-based
% %
% \par 
% %
% \textit{Learning-based methods.}
% %
% \MH{Todo}
% %


==> Sec/OLD_3_Method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Method} \label{sec:method}
%
\input{Fig/1_fig_method}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Put an overview figure here.
%
Todo
%
% Problem setting in one sentence
% Then step by step description of our method with reference to later chapters
% Next, we first describe our data assumptions and the notation
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par
%
\textbf{Data assumptions.}
%
% We assume $C$ camera views are given of a static or dynamic scene ....
%
Todo
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par
%
\textbf{Notation.}
%
% matrices are denoted as ... and so on
Todo
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\subsection{Background} \label{sec:background}
%%%%%%%%%% background %%%%%%%%%% 

\textbf{Background} \yiming{In this paragraph we briefly review the NeUS representation and Instant-ngp's hash grid representation.}
Given multi-view images of a static object and their camera parameters, NeuS~\cite{wang2021neus} reconstructs the 3D geometry of the object as a signed distance field $f$, and the geometry appearance as a radiance field $c$. Both $f$ and $c$ are encoded implicitly as multi-layer perceptions (MLPs). The signed distance field is represented as $f (x): \mathbb{R}^3 \to \mathbb{R}$, where $x$ is 3D position, and the radiance field $c (x, d):\mathbb{R}^3 \times \mathbb{S}^2 \to \mathbb{R}^3$ is parameterized by both 3D position $x$ and view direction $d \in \mathbb{S}^2$. The surface $\mathcal{S}$ of the object can be extracted by the zero-set of the signed distance function (SDF) values: $\mathcal{S} = \{x\in \mathbb{R}^3|f(x)=0\}$.

To render the object into an image, NeuS uses volume rendering. Different from a standard volume rendering which would result in geometric biases when associated with SDF, NeuS transforms the signed distance field into a volume density field by $\Phi_s(x)=1/(1+e^{-sx})$ ($s$ is a learnable parameter), and constructs an unbiased weight function in the volume rendering equation. Specifically, for each pixel of an image, we sample $n$ points $\{p(t_i)=o+t_id|i=0,1,\dots, n-1\}$ along its camera ray, where $o$ is the center of the camera and $d$ is the direction of the ray.
By accumulating the SDF-based densities and colors of the sample points, we can compute the color $\hat{C}$ of the ray as:

\begin{equation}
\hat{C} = \sum_{i=0}^{n-1} T(t_i)\alpha(t_i)c(t_i)
\end{equation}

where $T(t_i)$ is the discrete accumulated transmittances defined by $T(t_i)=\prod_{j=0}^{i-1}(1-\alpha(t_j))$, and $\alpha(t_i)$ is discrete density value defined by

\begin{equation} \label{eqn:neus_rendering_alpha}
\alpha(t_i) = \max\Big(\frac{\Phi_s(f(p(t_{i})))-\Phi_s(f(p(t_{i+1})))}{\Phi_s(f(p(t_{i})))}, 0\Big).
\end{equation}

As the rendering process is naturally differentiable, NeuS can learn the signed distance field $f$ and the radiance field $c$ from multi-view image input. However, the training process is very slow, taking about 15 hours for a static object on a single GPU. In this work, we propose a new method, \emph{NeuS2} to accelerate this process, which can achieve training in 40 seconds on a single GPU. We further develop an efficient training strategy for moving objects.
% Recent neural implicit representations, such as NeuS\cite{wang2021neus}, model the 3D geometry of an object as $f(\theta, x): \mathbb{R}^3 \to \mathbb{R}$ that maps a point $x \in \mathbb{R}^3$ to its signed distance to the geometry surface, where $\theta$ is learnable parameters. 
% The surface $\mathcal{S}$ of the object can be extracted by the zero-set of the SDF values: $\mathcal{S} = \{x\in \mathbb{R}^3|f(\theta, x)=0\}$. 
% This representation can be further rendered from novel views via volume rendering with the aid of the S-\textit{density} function $\Phi_s(x)=1/(1+e^{-sx})$ that transforms the signed distance field into a volume density field, with $s$ being a learnable parameter that gradually increases during training. 



To further achieve high efficiency and accuracy of 3D reconstruction, we utilize multi-resolution hash encodings $f_{\mathrm{enc}}(\theta_h, x)$ proposed by Instant-NGP\cite{muller2022instant_ngp}, which encode each point $x$ into spatial grids that are mapped to hash tables with learnable features $\theta_h$.
The $f_{\mathrm{enc}}(\theta_h, x)$ improves the capacity of neural geometry representations, which allows fast training using a smaller network without compromising quality.

Based on our neural geometry representation, an end-to-end and fast learning scheme can be achieved under the supervision of multi-view images.


\subsection{Efficient Neural Surface Reconstruction of Static Objects} \label{sec:method_static}


\yiming{In this part we introduce our method for static scene reconstruction.}



%%%%%%%%%% pipeline %%%%%%%%%% 
\textbf{NeuS2} 
\yiming{In this paragraph we demonstrate our pipeline that combines the NeuS representation with the hash grid. In detail, we illustrate the network structure, the geometry initialization method, the ray marching strategy, the loss function, and the implementation of the second-order derivative.}
As illustrated in Figure \ref{fig:overview}(a), we present \emph{NeuS2} for efficient and accurate static scene reconstruction from multi-view images. 
% It involves hash grid encoding technique proposed by~\cite{muller2022instant_ngp} with SDF-based volume rendering analogous to NeuS~\cite{wang2021neus}.
Given a query point $x \in \mathbb{R}^3$, we first obtain a set of feature vectors  $\{F_{hash}^i\}, F_{hash}^i\in \mathbb{R}^d $ from the $L$-level hash grids and concatenate them into the feature vector $F_{hash} \in \mathbb{R}^{L\times d}$ as part of our SDF network input.

\begin{equation} \label{eqn:hash_grid}
F_{hash}=f_\mathrm{enc}(x)
\end{equation}

Specifically, for each level, we identify the grids that correspond to the point $x$ and interpolate the learnable feature vectors of the grid vertices that are stored in the hash tables queried by vertex positions.
Additionally, we also feed the original query point $x$ into our SDF network to implement the geometry initialization proposed in SAL~\cite{atzmon2020sal} for our neural geometry representation. \yiming{whether to do? describe the benefits of the geometry initialization.}


The SDF network $f_\mathrm{sdf}$, consisting of a shallow MLP, outputs a SDF value $sdf$ of the query point and a geometry feature vector $F_\mathrm{geo}$, denoted as

\begin{equation} \label{eqn:sdf_net}
\begin{aligned}
x_\mathrm{enc} &= (x, F_{\mathrm{hash}}), \\
(sdf, F_\mathrm{geo}) &= f_\mathrm{sdf}(x_\mathrm{enc}).    
\end{aligned}
\end{equation}

Following NeuS~\cite{wang2021neus}, we compute the normal of the point as $n=\nabla_{\mathrm{x}}{sdf}$ and then combine it with the geometry feature $F_\mathbf{geo}$, the point $x$ and the ray direction $d$ as the input of our RGB network $f_\mathbf{rgb}$ to acquire predicted color $c_x$, which is formulated as

\begin{equation} \label{eqn:color_net}
c_x = f_\mathrm{rgb}(x, n, d, F_\mathrm{geo}).
\end{equation}

% As defined before, the gradients of the normal $n$ need to be backpropagated to the SDF as the second-order derivative, which will be discussed in detail later.

When conducting the volume rendering, we follow the ray marching strategy of Instant-NGP\cite{muller2022instant_ngp}.
That is, we maintain a cascade of multiscale occupancy grids to skip ray marching steps in empty space.
We periodically update the density grids based on the SDF value predicted by our model.

To optimize the neural geometry and appearance representations simultaneously, we utilize the following loss function that minimizes the discrepancy between rendered pixel colors and the ground truth as well as regularizes the signed distance field
\begin{equation} \label{eqn:loss}
    \mathcal{L}=\mathcal{L}_{\mathrm{color}}+\beta \mathcal{L}_{\mathrm{eikonal}},
\end{equation}
where we assume the number of the sample points along a ray is $n$ and the batch size is $m$. 
The color loss $\mathcal{L}_{\mathrm{color}}$ is defined as 
\begin{equation} \label{eqn:color_loss}
    \mathcal{L}_{\mathrm{color}} = \frac{1}{m}\sum_{i} \mathcal{R}(\hat{C_i}, C_i).
\end{equation}

Similar to Instant-NGP\cite{muller2022instant_ngp}'s implementation, we set $\mathcal{R}$ as Huber loss to achieve a more efficient and stable training process.

The Eikonal loss~\cite{gropp2020igr} $\mathcal{L}_{\mathrm{eikonal}}$ is defined as
\begin{equation} \label{eqn:eikonal_loss}
    \mathcal{L}_{\mathrm{eikonal}} = \frac{1}{mn}\sum_{k,i}(|n_{k,i}|-1)^2.
\end{equation}



% \yiming{Formula of the second-order derivative: we organize the derivation as this: 1. Chain rules for second-order derivative; 2. Application of the the chain rule to the MLP and the MLP's second-order derivative formula} 

\textbf{CUDA implementation} Similar to Instant-NGP~\cite{muller2022instant_ngp}, we implement our system in CUDA, based on the \textit{tiny-cuda-nn}~\cite{tiny-cuda-nn} framework. To train our model, we first calculate the gradients of the model's parameters, including the hash table $f_\mathrm{enc}$, the SDF network $f_\mathrm{sdf}$, and the RGB network $f_\mathrm{rgb}$ and then optimize the parameters by using the Adam~\cite{Adam} optimizer. Different from Instant-NGP, which only needs to calculate the first-order gradients during the optimization, we also need to calculate the second-order gradients to optimize our model on account of the normal term $n=\nabla_{\mathrm{x}}{sdf}$ used in the input of the RGB network $f_\mathrm{rgb}$~\ref{eqn:color_net}, the Eikonal loss term $\mathcal{L}_{\mathrm{eikonal}}$~\ref{eqn:eikonal_loss}, and the NeuS rendering procedure~\ref{eqn:neus_rendering_alpha}.

To accelerate the gradients calculation progress, we directly calculate the second-order gradients by using the chain rule instead of applying the computation graph used in Pytorch~\cite{NEURIPS2019_9015pytorch}. Specifically, we calculate the second-order gradients of the hash table parameters $\theta_\mathrm{enc}$ and the SDF network parameters $\theta_\mathrm{sdf}$ from $\frac{\partial \mathcal{L}}{\partial n}$ by using the chain rule. Note that the RGB network $f_\mathrm{rgb}$ only takes $n$ as input, so we don't have to calculate its second-order gradients. Following the network structure defined in~\ref{eqn:hash_grid}, ~\ref{eqn:sdf_net}, we have:

% (For simplicity, we define $enc = (x, F_{\mathrm{hash}})$)  

\begin{equation} \label{eqn:dloss_denc}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \theta_\mathrm{enc}}(n)
& = \frac{\partial \mathcal{L}}{\partial n} \frac{\partial \frac{\partial sdf}{\partial x}}{\partial \theta_\mathrm{enc}} \\
&= \frac{\partial \mathcal{L}}{\partial n} \frac{\partial (\frac{\partial sdf}{\partial x_\mathrm{enc}} \frac{\partial x_\mathrm{enc}}{\partial x})}{\partial \theta_\mathrm{enc}} \\
&= \frac{\partial \mathcal{L}}{\partial n} (
\frac{\partial x_\mathrm{enc}}{\partial x} \frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial \theta_\mathrm{enc}}
+ \frac{\partial sdf}{\partial x_\mathrm{enc}} \frac{\partial \frac{\partial x_\mathrm{enc}}{\partial x}}{\partial \theta_\mathrm{enc}}
) \\
&= \frac{\partial \mathcal{L}}{\partial n} (
\frac{\partial x_\mathrm{enc}}{\partial x} \frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial x_\mathrm{enc}} \frac{\partial x_\mathrm{enc}}{\partial \theta_\mathrm{enc}}
+ \frac{\partial sdf}{\partial x_\mathrm{enc}} \frac{\partial \frac{\partial x_\mathrm{enc}}{\partial x}}{\partial \theta_\mathrm{enc}}
)
\end{aligned}
\end{equation}

Similarly, we have
\begin{equation} \label{eqn:dloss_dsdf}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \theta_\mathrm{sdf}}(n) 
&= 
\frac{\partial \mathcal{L}}{\partial n} (
\frac{\partial x_\mathrm{enc}}{\partial x} \frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial \theta_\mathrm{sdf}} 
+ \frac{\partial sdf}{\partial x_\mathrm{enc}} \frac{\partial \frac{\partial x_\mathrm{enc}}{\partial x}}{\partial \theta_\mathrm{sdf}}
)
% \\&= \frac{\partial \mathcal{L}}{\partial n} \frac{\partial enc}{\partial x} \frac{\partial \frac{\partial sdf}{\partial enc}}{\partial \theta_\mathrm{sdf}} 
\end{aligned}
\end{equation}

Based on the equations \ref{eqn:dloss_denc} and \ref{eqn:dloss_dsdf}, the second-order gradients can be calculated by the second-order derivative formula of the hash grid $f_\mathrm{enc}$ and the SDF network $f_\mathrm{sdf}$, including $ \frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial x_\mathrm{enc}}, \frac{\partial \frac{\partial x_\mathrm{enc}}{\partial x}}{\partial \theta_\mathrm{enc}}, \frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial \theta_\mathrm{sdf}}$. We implement the second-order derivative of ReLU based MLP in CUDA for the SDF network and use the second-order derivative implementation in \textit{tiny-cuda-nn} for the hash grid. 

% \textbf{Theorem 1} (The second-order derivative of the MLP) \label{second_order_derivative}
% Given a \textit{ReLU} based MLP $f$ with $L$ hidden layers taking $x \in \mathbb{R}^{d}$ as input, it layer-wisely computes $x_l = R(H_lx_{l-1})$, where $l\in \{1,\dots,L\}$ is the layer index, $x_0 = x$, $ x_l \in \mathbb{R}^{n_l}$, $H_l \in \mathbb{R}^{n_l \times n_{l-1}}$ and $R$ is the ReLU function. The second-order derivative formula of the MLP $f$ is:
% \begin{equation}
% \frac{\partial \frac{\partial y}{\partial x}}{\partial H_l} = (H_{l+1}^T \dots RH_L^TS_L) (H_{l-1} \dots RH_1S_1)
% % d(dy\_dx)\_d(H^i_{mn}) = 
% % \Sigma_k \{H^1 R H^2 \dots R H^{i-1} R\}_{kn} * \Sigma_l \{RH^{i+1} \dots RH^n\}_{ml}
% \end{equation}

% \begin{equation}
% \frac{\partial^2 y}{\partial \mathbf{x}^2} = 0
% \end{equation}



\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}

\begin{definition} \label{def:mlp}
Given a ReLU based MLP $f$ with $L$ hidden layers taking $x \in \mathbb{R}^{d}$ as input, it computes the output $y = H_L g(H_{L-1} \dots g(H_1x))$, where $H_l \in \mathbb{R}^{n_l} \times \mathbb{R}^{n_{l-1}}$, $l\in \{1,\dots,L\}$ is the layer index, and $g$ is the ReLU function. We define $P_l^j \in \mathbb{R}^{n_{l-1}} \times \mathbb{R}^1 $ and $S_l^i \in \mathbb{R}^ 1 \times \mathbb{R}^{n_{l}}$ as


\begin{equation}
\begin{aligned}
P_l &= G_{l-1} H_{l-1} \dots G_1 H_1^{(\_,j)} \\ 
S_l &= H_L^{(i,\_)} G_{L-1} \dots H_{l+1} G_{l+1}
% S_l &= H_{l+1} \dots g(H_L^{(i,\_)})
\end{aligned}
\end{equation}
where $H_1^{(\_,j)}$ means the $ j$ th  column of $H_1$, 
$H_L^{(i, \_)}$ means the $ i$ th row of $H_L$, and
$G_l = g(H_{l-1}x_{l-1})$.

\end{definition}



\begin{theorem} [The second-order derivative of MLP]
Given a ReLU based MLP $f$ with $L$ hidden layers with the same definition in \ref{def:mlp}. The second-order derivative formula of the MLP $f$ is:
\begin{equation}
\begin{aligned}
\frac{\partial \frac{\partial y}{\partial x}_{(i,j)}}{\partial H_l} & = (P_l^i S_l^j)^T
% \frac{\partial \frac{\partial y}{\partial x}}{\partial H_l} = (H_{l+1}^T \dots g(H_L^TS_L)) (H_{l-1} \dots g(H_1S_1))
% d(dy\_dx)\_d(H^i_{mn}) = 
% \Sigma_k \{H^1 R H^2 \dots R H^{i-1} R\}_{kn} * \Sigma_l \{RH^{i+1} \dots RH^n\}_{ml}
\end{aligned}
\end{equation}

\begin{equation}
\frac{\partial^2 y}{\partial \mathbf{x}^2} = 0
\end{equation}

% where $S_l$ and $P_l$ are the prefix product and suffix product defined in \ref{def:mlp}, and $S_l P_l^T$ means the matrix multiplication from matrix with dimension $\mathbb{R}^{n_l} \times 1$ and matrix with dimension $1 \times \mathbb{R}^{n_{l-1}}$ to the matrix with dimension $\mathbb{R}^{n_l} \times \mathbb{R}^{n_{l-1}}$.
% \end{theorem}

where $S_l^j$ and $P_l^i$ are defined in \ref{def:mlp}.
\end{theorem}

The proof is given in the supplementary material. 
From the properties of the hash grid and the SDF network's second-order derivative, we know that $\frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial x_\mathrm{enc}} = 0$ and $\frac{\partial \frac{\partial x_\mathrm{enc}}{\partial x}}{\partial \theta_\mathrm{sdf}} = 0$, which helps us to simplify the equations \ref{eqn:dloss_denc} and \ref{eqn:dloss_dsdf} to
% We can use the properties of the hash grid and the SDF network's second-order derivative to simplify the equations \ref{eqn:dloss_denc} and \ref{eqn:dloss_dsdf} as:

\begin{equation} \label{eqn:simplified_dloss_denc}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \theta_\mathrm{enc}} (n)
&= \frac{\partial \mathcal{L}}{\partial n} \frac{\partial sdf}{\partial x_\mathrm{enc}} \frac{\partial \frac{\partial x_\mathrm{enc}}{\partial x}}{\partial \theta_\mathrm{enc}}
\end{aligned}
\end{equation}

\begin{equation} \label{eqn:simplified_dloss_dsdf}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \theta_\mathrm{sdf}} (n)
&= 
\frac{\partial \mathcal{L}}{\partial n} 
\frac{\partial x_\mathrm{enc}}{\partial x} \frac{\partial \frac{\partial sdf}{\partial x_\mathrm{enc}}}{\partial \theta_\mathrm{sdf}} 
% \\&= \frac{\partial \mathcal{L}}{\partial n} \frac{\partial enc}{\partial x} \frac{\partial \frac{\partial sdf}{\partial enc}}{\partial \theta_\mathrm{sdf}} 
\end{aligned}
\end{equation}

By using this final form of the second-order gradients, we can avoid some unnecessary calculation and thus improve efficiency.
% Given the loss function $\mathcal{L}$, we optimize the parameters hash grids calculate the second-order gradient of the hash grids $\vect{F_{hash}}$ and the SDF network $f_\mathrm{sdf}$ based on the chain rule of derivatives.

% \textbf{Lemma 1} (Chain rules for second-order derivative) \label{second_order_derivative}
% Suppose two networks $f_1(\mathbf{\theta_1}), f_2(\mathbf{\theta_2})$, where $\theta_1$ and $\theta_2 $ are the network's learnable parameters, are combined to form a mapping $f = f_2 \cdot f_1 $. Given an input $ \mathbf{x}$, the network computes $f(\mathbf{x}) = f_2( f_1(\mathbf{x}))$. We denote $ y_1 = f_1(x)$ and $y_2 = f_2(y_1)$. For a loss function $L$ that is relevant to the gradient term $\nabla_{\mathrm{\mathbf{x}}}{f}$, e.g. the Eikonal loss $\left(\left\|\nabla_{\mathrm{\mathbf{x}}}{f} \right\|_2-1\right)^2 $, the second-order derivatives according to $\mathbf{x}, \mathbf{\theta_1}, \mathbf{\theta_2}$ are:


% \begin{equation}
% \frac{\partial^2 L}{\partial \mathbf{x}^2} =
% \end{equation}

% \begin{equation}
% \frac{\partial^2 L}{\partial \mathbf{\theta_1}^2} =
% \end{equation}

% \begin{equation}
% \frac{\partial^2 L}{\partial \mathbf{\theta_2}^2} =
% \end{equation}





\textbf{Progressive training} \yiming{In this paragraph we introduce the progressive training method, which gradually increases the bandwith of the hash grid.} We implement a coarse-to-fine optimization process for multi-resolution spatial encoding to learn the neural implicit representation more stable and robust.
We observe from the experiments that using grids with small resolutions results in under-fitting of the data, in which the geometry reconstruction result is smooth and lacking details, whereas grids with large resolutions induces over-fitting, leading to increased noise and artifacts of the results.
Therefore, we conduct a progressive training method by gradually increasing the bandwidth of our spatial grid encoding denoted as:
\begin{equation}
   f_\mathrm{enc}(x, \lambda) = \big(w_0(\lambda) F_{\mathrm{hash}}^0, \dots, w_{L-1}(\lambda) F_{\mathrm{hash}}^{L-1}\big), 
\end{equation}
% enc(\theta, x, \lambda) = \big(w_0(\lambda) F_0(x), w_1(\lambda) F_2(x), \dots, w_{L-1}(\lambda) F_{L-1}(x)\big),
where the weight $w_i$ for each grid encoding level is defined by
\begin{equation}
w_i(\lambda)=
\begin{cases}
0, \text{ if } i>\lambda \\
1, \text{ otherwise} 
\end{cases},
\end{equation}
and the parameter $\lambda$ can be interpreted as a controller of the bandwidth of the low-pass filter applied to the multi-resolution grid encoding, which gradually increases during the training process.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Fast Reconstruction of Moving Objects} \label{sec:method_dynamic}

In this section, we present our fast dynamic geometry reconstruction pipeline, involving frame-by-frame incremental training and global transformation prediction.


\textbf{Incremental training} \hanqin{In this paragraph we demonstrate our incremental training method.}
Even though our static scene 3D reconstruction can achieve promising efficiency and quality, constructing dynamic scene by training every single frame independently is still time-consuming.
An incremental training strategy is thus proposed to exploit the geometry and appearance representation similarity sharing between two adjacent frames that enable faster convergence of our model.
In detail, we train the first frame from scratch as illustrated in our static scene reconstruction, and then fine-tune the model's parameters for subsequent frames based on the learned representation of the previous frame.
Using this strategy, the model is able to establish a feasible initialization of the target representation that significantly accelerates its convergence speed.



\textbf{Global transformation prediction} \hanqin{In this paragraph we demonstrate our global movement prediction implementation, including: 1. learning obstacles (stuck in local minima) faced with large movement, like walking; 2. proposed end-to-end global rotation & transition prediction strategy and corresponding formula.}
As we observed during incremental training process, some regions, which are occluded in some views, of the predicted SDF may get stuck in the learned SDF of the previous frame as the local minima, when the object's movement between adjacent frames is relatively large.
For instance, when our model reconstructs a walking sequence from muli-view images, the reconstructed surface appears to have many holes.
% This phenomenon is caused by 
% since our 
% only relies on 
To address this issue, we propose a global transformation prediction to roughly transform the target SDF into canonical space before incremental training.
Specifically, we predict the rotation $R$ and transition $T$ of the object between two adjacent frames. For any given point $X_i$ in the coordinate space of the frame $i$, it is transformed back to the coordinate space of the previous frame $i-1$, defined as $X_{i-1}$
\begin{equation} \label{eqn:globalmove_predict}
    X_{i-1}=R_i(X_{i}+T_i).
\end{equation}
The transformations can then be accumulated to transform the point $X_i$ back to $X_c$ in the first frame's coordinate space
\begin{equation}
    X_c=R_{i-1}^c(X_{i-1}+T_{i-1}^c)=R_{i}^c(X_{i}+T_{i}^c),
\end{equation}
where $R_i^c=R_{i-1}^cR_i$ and $T_i^c=T_i+R_i^{-1}T_{i-1}^c$.
Note that this transformation definition~\ref{eqn:globalmove_predict} explicitly separates the rotation from transition, compared with another form $X_{i-1}=R_iX_{i}+T_i$, which enables better learning efficiency and accuracy.

We achieve our incremental training combined with global transformation prediction as an end-to-end learning scheme, as illustrated in figure~\ref{fig:overview}(b). When turning to a new frame, we first predict the global transformation independently, and after reaching training convergence for the global prediction, we fine-tune the model's parameters and global transformation together to efficiently learn the neural representation.

%

==> Sec/OLD_3_Method_new.tex <==
%%%%%%%%%%%%
\input{Fig/1_fig_method}
%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
\section{Background} \label{sec:background}
%
%%%%%%%%%%%%
%
\textbf{Surface Representation.}
%
The surface and appearance of a scene can be implicitly represented as a signed distance field $f (\mathbf{x}): \mathbb{R}^3 \to \mathbb{R}$, where $\mathbf{x}$ is a 3D position, and a radiance field $c (\mathbf{x}, \mathbf{v}):\mathbb{R}^3 \times \mathbb{S}^2 \to \mathbb{R}^3$.
%
Here, $\mathbf{x}$ denotes a 3D position and $\mathbf{v} \in \mathbb{S}^2$ is a viewing direction. 
%
The surface $\mathcal{S}$ of the object can be obtained by extracting the zero-level set of the signed distance function (SDF) $\mathcal{S} = \{\mathbf{x}\in \mathbb{R}^3|f(\mathbf{x})=0\}$.
%
%%%%%%%%%%%%
%
\par
%
\textbf{NeuS.} 
%
Given calibrated multi-view images of a static scene, NeuS~\cite{wang2021neus} implicitly reconstructs the 3D geometry of the object as such a signed distance field $f$, and the appearance as a radiance field $c$. 
%
Both $f$ and $c$ are encoded as multi-layer perceptions (MLPs). 
%
To render an object into an image, NeuS leverages volume rendering. 
%
However, naively using the SDF values as a density function in the rendering formulation would introduce a bias to the reconstructed geometry.
%
Instead, NeuS first transforms the signed distance field into a volume density field $\phi_s(f(\textbf{x}))$, where $\phi_s(x)=se^{-sx}/(1+e^{-sx})^2$ is the \textit{logistic density distribution}, which is the derivative of the Sigmoid function $\Phi_s(x)=1/(1+e^{-sx})$ and $s$ is a learnable parameter.
%
Next, NeuS constructs an unbiased weight function in the volume rendering equation. 
%
Specifically, for each pixel of an image, we sample $n$ points $\{\mathbf{\mathbf{p}(t_i)}=\mathbf{o}+t_i\mathbf{v}|i=0,1,\dots, n-1\}$ along its camera ray, where $\mathbf{o}$ is the center of the camera and $\mathbf{v}$ is the view direction.
%
By accumulating the SDF-based densities and colors of the sample points, we can compute the color $\hat{C}$ of the ray with the same approximation scheme as used in NeRF~\cite{mildenhall2020nerf} as
%
%%%%%%%%%%%%
\begin{equation}
\hat{C}(\mathbf{o}, \mathbf{v}) = \sum_{i=0}^{n-1} T({t_i})\alpha({t_i})c(\mathbf{p}({t_i}), \mathbf{v})
\label{eqn:neus_volume_rendering}
\end{equation}
%%%%%%%%%%%%
%
where $T(t_i)$ is the discrete accumulated transmittance defined by $T(t_i)=\prod_{j=0}^{i-1}(1-\alpha(t_j))$, and $\alpha(t_i)$ is a discrete density value defined by
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:neus_rendering_alpha}
\alpha(t_i) = \max\Big(\frac{\Phi_s(f(p(t_{i})))-\Phi_s(f(p(t_{i+1})))}{\Phi_s(f(p(t_{i})))}, 0\Big).
\end{equation}
%%%%%%%%%%%%
%
As the rendering process is differentiable, NeuS can learn the signed distance field $f$ and the radiance field $c$ from the multi-view images. 
%
However, the training process is very slow, taking about 8 hours for a static object on a single GPU. 
%
%%%%%%%%%%%%
%
\par 
%
\textbf{Multi-resolution Hash Encoding.} 
%
To overcome the slow training time of deep coordinate-based MLPs, which are also one of the main reasons for the slow performance of NeuS, recently, instant-NGP~\cite{muller2022instant_ngp} proposed a multi-resolution hash encoding and has proven its effectiveness.
%
Specifically, instant-NGP assumes the object to be reconstructed is bounded in multi-resolution voxel grids. 
%
The voxel grids at each resolution map to a hash table with a fixed-size array of learnable feature vectors.
%
For a 3D position $\mathbf{x} \in \mathbb{R}^3$, it obtains a hash encoding at each level $h^i (\mathbf{x})\in \mathbb{R}^d$ (d is the dimension of a feature vector, $i=1, ..., L$) by interpolating the feature vectors assigned at the surrounding voxel grids at this level. 
%
The hash encodings at all $L$ levels are then concatenated to be the multi-resolution hash encoding $h(\mathbf{x}) =\{h^i(\mathbf{x})\}_{i=1}^{L}\in \mathbb{R}^{L\times d}$.
%
While the runtime is significantly improved, instant-NGP still does not reach the quality of NeuS in terms of geometry reconstruction accuracy.
%
%%%%%%%%%%%%
%
\par 
%
\textbf{Discussion.}
%
Given the above discussion, one can ask whether a naive combination of an implicit surface representation, the hash encoding, and the unbiased rendering formulation of NeuS can unite the best of the two worlds, i.e. high 3D surface reconstruction quality \textit{and} efficient computation.
%
We found that uniting these concepts is far from being trivial and novel challenges arise that require dedicated design choices resulting in our proposed approach, called \textit{NeuS2}.
%
Next, we describe how NeuS2 can achieve a high quality reconstruction of a static scene in under 40 seconds on a single GPU (Sec.~\ref{sec:method_static}). 
%
Afterwards, we further extend our static formulation to the dynamic case where we reconstruct dynamic scenes, i.e. depicted by multi-view \textit{videos}, in a highly efficient manner (Sec.~\ref{sec:method_dynamic}).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
\section{Static Neural Surface Reconstruction} \label{sec:method_static}
%
We first present how our formulation can effectively learn the signed distance field of a \textit{static} scene from calibrated multi-view images (see Fig.~\ref{fig:overview} a)). 
%
To accelerate the training process, we first demonstrate how to incorporate multi-resolution hash encodings~\cite{muller2022instant_ngp} for representing the SDF of the scene, and how unbiased volume rendering can be applied to render the scene into an image (Sec~\ref{sec:representation}). 
%
Now, when the unbiased volume rendering and the respective regularization should be applied for supervision, second-order derivates have to be computed.it is 
%
A naive implementation, however, would be too slow (as demonstrated in our experiments). 
%
Thus, we derive an efficient computation of second-order derivatives tailored to ReLU-based MLPs, which can be efficiently parallelized in custom CUDA kernels (Sec~\ref{sec:derivatives}). 
%
Finally, we introduce a progressive training strategy for learning multi-resolution hash encodings, which leads to faster training convergence and better reconstruction quality (Sec~\ref{sec:progessive}). 
%
%%%%%%%%%%%%
%
\subsection{Unbiased Rendering of a Hash-encoded SDF} \label{sec:representation}
%
For each 3D position $\mathbf{x}$, we map it to its multi-resolution hash encodings $h_\Omega(\mathbf{x})$ with learnable hash table entries $\Omega$.
%
As $h_\Omega(\mathbf{x})$ is an informative encoding of spatial position, the MLPs for mapping $\mathbf{x}$ to its SDF $d$ and color $c$ can be very shallow , which results in more efficient rendering and training without compromising quality.
%
%%%%%%%%%%%%
%
\par
\textbf{SDF Network.}
%
In more detail, our SDF network 
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:sdf_net}
\begin{aligned}
(d, \mathbf{g}) &= f_{\Theta}(\mathbf{e}), \\   
\mathbf{e} &= (\mathbf{x}, h_\Omega(\mathbf{x})).
\end{aligned}
\end{equation}
%%%%%%%%%%%%
%
is a shallow MLP, which takes the 3D position $\mathbf{x}$ along with its hash encoding $h_\Omega(\mathbf{x})$ as input and outputs the SDF value $d$ and a geometry feature vector $\mathbf{g} \in \mathbb{R}^{15}$.
%
Concatenating the position serves as a geometry initialization~\cite{atzmon2020sal} leading to a more stable learning of the geometry. 
%
Here, $\Theta$ are the trainable network parameters. 
%
%%%%%%%%%%%%
%
\par
\textbf{Color Network.}
%
The normal of the point $\mathbf{x}$ can be computes as 
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:normal}
\mathbf{n}=\nabla_{\mathbf{x}}d.
\end{equation}
%%%%%%%%%%%%
%
where $\nabla_{\mathbf{x}}d$ denotes the gradient of the SDF with respect to $\mathbf{x}$.
%
We then combine the normal with the geometry feature $\mathbf{g}$, the point $\mathbf{x}$, and the ray direction $\textbf{v}$ serving as the input to our color network
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:color_net}
\mathbf{c} = c_{\Upsilon}(\textbf{x}, \textbf{n}, \textbf{v}, d, \mathbf{g}),
\end{equation}
%%%%%%%%%%%%
%
which predicts the color $\mathbf{c}$ of $\mathbf{x}$. 
%
%%%%%%%%%%%%
%
\par
\textbf{Unbiased Scene Rendering.}
%
To render an image, we apply the unbiased volume rendering of NeuS~\cite{wang2021neus} (see Eq. \ref{eqn:neus_volume_rendering}, \ref{eqn:neus_rendering_alpha}).
%
Additionally, we adopt a ray marching acceleration strategy used in Instant-NGP\cite{muller2022instant_ngp}.
%
That is, we maintain an occupancy grid that roughly marks each voxel grid as empty or non-empty.
%
The occupancy grid can effectively guide the marching process by preventing sampling in empty spaces and, thus, accelerate the volume rendering process.
%
We periodically update the occupancy grid based on the SDF value predicted by our model. In detail, we first use the SDF value $d$ to calculate the density value $\phi_s(d)$ for each grid, where $\phi_s(x)=se^{-sx}/(1+e^{-sx})^2$ is the \textit{logistic density distribution} and $s$ is a learnable parameter. We then use the density value to update the occupancy grid in the same way as Instant-NGP\cite{muller2022instant_ngp}. \LJ{give an equation? \yiming{finished}}.

%
%%%%%%%%%%%%
%
\par
\textbf{Supervision.}
%
To train NeuS2, we minimize the color difference between the rendered pixels $\hat{C_i}$ with $i \in \{1,...,m\}$ and the corresponding ground truth pixels ${C_i}$ without any 3D supervision. 
%
Here, $m$ denotes the batch size during training.
%
We also employ an Eikonal term~\cite{gropp2020igr} to regularize the learned signed distance field leading to our final loss
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:loss}
    \mathcal{L}=\mathcal{L}_{\mathrm{color}}+\beta \mathcal{L}_{\mathrm{eikonal}},
\end{equation}
%%%%%%%%%%%%
%
where
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:color_loss}
    \mathcal{L}_{\mathrm{color}} = \frac{1}{m}\sum_{i} \mathcal{R}(\hat{C_i}, C_i),
\end{equation}
%%%%%%%%%%%%
\begin{equation} \label{eqn:eikonal_loss}
    \mathcal{L}_{\mathrm{eikonal}} = \frac{1}{mn}\sum_{k,i}(||\mathbf{n}_{k,i}||-1)^2.
\end{equation}
%%%%%%%%%%%%
%
$\mathcal{R}$ is the Huber loss~\cite{huber}.
%
$k$ indexes the $k$th sample along the ray with $k \in \{1,...,n\}$, and $n$ is the number of sampled points.
%
$\mathbf{n}_{k,i}$ is the normal of a sampled point (see Eq.~\ref{eqn:normal}). 
%
\par 
%
Importantly, the rendering formulation of NeuS as well as the Eikonal loss operate on the normal, i.e., the gradient of the SDF value with respect to the position $\mathbf{x}$.
%
Thus, during backpropagation the second-order derivates are required as well, which are, however, expensive to compute when using the standard auto differentation tools offered by most deep learning frameworks.
%
%%%%%%%%%%%%
%
\subsection{Efficient Handling of Second-order Derivatives} \label{sec:derivatives}
%
To avoid the computational overhead that learning frameworks such as PyTorch introduce, for example  by constructing the computational graph, we implement our whole system in CUDA, based on the \textit{tiny-cuda-nn}~\cite{tiny-cuda-nn} framework. 
%
For backpropagation, we first calculate the first-order derivatives of the model parameters including the hash table entries $\Omega$, the SDF network weights $\Theta$, and the RGB network weights $\Upsilon$.
%
We leverage the Adam~\cite{Adam} optimizer throughout the training process. 
%
%%%%%%%%%%%%
%
\par
%
\textbf{Second-order Derivative Computation.}
%
In stark contrast to Instant-NGP~\cite{muller2022instant_ngp}, which only requires the first-order derivatives during the optimization, we also have to calculate the second-order derivatives for the parameters associated with the normal term $\mathbf{n}=\nabla_{\mathrm{x}}d$ (Eq.~\ref{eqn:normal}), which is used as an input to the color network $c_\Upsilon$ (Eq.~\ref{eqn:color_net}) and the Eikonal loss term $\mathcal{L}_{\mathrm{eikonal}}$ (Eq.~\ref{eqn:eikonal_loss}).
%
To accelerate the calculation of the second-order derivatives, we directly calculate them using the chain rule instead of applying the computation graph used in Pytorch~\cite{NEURIPS2019_9015pytorch}. 
%
Specifically, we calculate the second-order derivatives of the hash table parameters $\Omega$ as
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:dloss_denc}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \Omega}
& = \frac{\partial \mathcal{L}}{\partial \mathbf{n}} \frac{\partial \frac{\partial d}{\partial \mathbf{x}}}{\partial \Omega} \\
&= \frac{\partial \mathcal{L}}{\partial \mathbf{n}} \frac{\partial (\frac{\partial d}{\partial \mathbf{e}} \frac{\partial \mathbf{e}}{\partial \mathbf{x}})}{\partial \Omega} \\
&= \frac{\partial \mathcal{L}}{\partial \mathbf{n}} (
\frac{\partial \mathbf{e}}{\partial \mathbf{x}} \frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \Omega}
+ \frac{\partial d}{\partial \mathbf{e}} \frac{\partial \frac{\partial \mathbf{e}}{\partial \textbf{x}}}{\partial \Omega}
) \\
&= \frac{\partial \mathcal{L}}{\partial \mathbf{n}} (
\frac{\partial \mathbf{e}}{\partial \mathbf{x}} \frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \mathbf{e}} \frac{\partial \mathbf{e}}{\partial \Omega}
+ \frac{\partial d}{\partial \mathbf{e}} \frac{\partial \frac{\partial \mathbf{e}}{\partial \mathbf{x}}}{\partial \Omega}
)
\end{aligned}
\end{equation}
%%%%%%%%%%%%
%
and the SDF network parameters $\Theta$ as
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:dloss_dsdf}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \Theta} 
&= 
\frac{\partial \mathcal{L}}{\partial \mathbf{n}} (
\frac{\partial \mathbf{e}}{\partial \mathbf{x}} \frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \Theta} 
+ \frac{\partial d}{\partial \mathbf{e}} \frac{\partial \frac{\partial \mathbf{e}}{\partial \mathbf{x}}}{\partial \Theta}
)
\end{aligned}
\end{equation}
%%%%%%%%%%%%
%
using the chain rule. 
%
Note that the color network $c_\Upsilon$ only takes $\mathbf{n}$ as input, so we do not need to calculate its second-order gradients of the color network parameters $\Upsilon$. 
%
The derivation of Eq.~\ref{eqn:dloss_dsdf} is included in the supplemental document.
%
Based on Eq.~\ref{eqn:dloss_denc} and Eq.~\ref{eqn:dloss_dsdf}, the second-order gradients can be calculated by the second-order derivative formula of the hash grid $h$ and the SDF network $f_\Theta$, including $ \frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \mathbf{e}}, \frac{\partial \frac{\partial \mathbf{e}}{\partial \mathbf{x}}}{\partial \Omega}, \frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \Theta}$. 
%
%%%%%%%%%%%%
%
\par
%
To speed up the computation of Eq.~\ref{eqn:dloss_denc} and Eq.~\ref{eqn:dloss_dsdf}, we found that ReLU-based MLPs can greatly simplify the above terms leading to less computation overhead.
%
In the following, we discuss this in more detail and provide a complete proof of this proposition in the supplemental document. 
%
Therefore, we first introduce some useful definitions as follows.
%
\newtheorem{theorem}{Theorem}
%
\newtheorem{definition}{Definition}
%


%%%%%%%%%%%%
\begin{definition} \label{def:mlp}
% Given a ReLU based MLP $f$ with $L$ hidden layers taking $x \in \mathbb{R}^{d}$ as input, it computes the output $y = H_L g(H_{L-1} \dots g(H_1x))$, where $H_l \in \mathbb{R}^{n_l} \times \mathbb{R}^{n_{l-1}}$, $l\in \{1,\dots,L\}$ is the layer index, and $g$ is the ReLU function. 
% %
% We define $P_l^j \in \mathbb{R}^{n_{l-1}}$ and $S_l^i \in \mathbb{R}^{n_{l}}$ as
% %

Given a ReLU based MLP $f$ with $L$ hidden layers taking $x \in \mathbb{R}^{d}$ as input, it computes the output $y = H_L g(H_{L-1} \dots g(H_1x))$, where $H_l \in \mathbb{R}^{n_l} \times \mathbb{R}^{n_{l-1}}$, $l\in \{1,\dots,L\}$ is the layer index, and $g$ is the ReLU function. 
%
We define $P_l^j \in \mathbb{R}^{n_{l-1}} \times \mathbb{R}^1 $ and $S_l^i \in \mathbb{R}^ 1 \times \mathbb{R}^{n_{l}}$ as
%

%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
P_l &= G_{l-1} H_{l-1} \dots G_1 H_1^{(\_,j)} \\ 
S_l &= H_L^{(i,\_)} G_{L-1} \dots H_{l+1} G_{l+1}
\end{aligned}
\end{equation}
%%%%%%%%%%%%
%
% where $H_1^{(\_,j)}$ means the $ j$ th  column of $H_1$, $H_L^{(i, \_)}$ means the $ i$ th row of $H_L$, and $G_l = \frac{\partial g(H_{l-1}x_{l-1})}{\partial H_{l-1}x_{l-1}}$\yiming{Write $G_l$ in somewhat simpler form}.
where $H_1^{(\_,j)}$ means the $ j$ th  column of $H_1$, $H_L^{(i, \_)}$ means the $ i$ th row of $H_L$, and 
$G_l=
\begin{cases}
1, H_{l-1}\dots g(H_1x) > 0 \\
0, \text{ otherwise} 
\end{cases}$.
\end{definition}
%
Given the above definitions, the second order derivates of a ReLU-based MLP with respect to its input and intermediate layers can be defined as follows.
%
%%%%%%%%%%%%
\begin{theorem} [Second-order derivative of ReLU-based MLP] \label{theorem:mlp_derivative}
Given a ReLU based MLP $f$ with $L$ hidden layers with the same definition in Definition~\ref{def:mlp}. The second-order derivative formula of the MLP $f$ is:
\begin{equation}
\begin{aligned}
\frac{\partial \frac{\partial y}{\partial x}_{(i,j)}}{\partial H_l} & = (P_l^j S_l^i)^T
% \frac{\partial \frac{\partial y}{\partial x}}{\partial H_l} & =  S_l P_l^T
% \frac{\partial \frac{\partial y}{\partial x}}{\partial H_l} = (H_{l+1}^T \dots g(H_L^TS_L)) (H_{l-1} \dots g(H_1S_1))
% d(dy\_dx)\_d(H^i_{mn}) = 
% \Sigma_k \{H^1 R H^2 \dots R H^{i-1} R\}_{kn} * \Sigma_l \{RH^{i+1} \dots RH^n\}_{ml}
\end{aligned}
\end{equation}
\begin{equation}
\frac{\partial^2 y}{\partial \mathbf{x}^2} = 0
\end{equation}

where $\frac{\partial y}{\partial x}_{(i,j)}$ means the matrix element (i,j) of $\frac{\partial y}{\partial x}$, and $S_l^i$ and $P_l^j$ are defined in Definition \ref{def:mlp}.
% where $S_l$ and $P_l$ are the prefix product and suffix product defined in \ref{def:mlp}, and $S_l P_l^T$ means the matrix multiplication from matrix with dimension $\mathbb{R}^{n_l} \times 1$ and matrix with dimension $1 \times \mathbb{R}^{n_{l-1}}$ to the matrix with dimension $\mathbb{R}^{n_l} \times \mathbb{R}^{n_{l-1}}$.
\label{theo}
\end{theorem}
%%%%%%%%%%%%
%
Coming back to our original second-order derivatives (Eq.~\ref{eqn:dloss_denc} and Eq.~\ref{eqn:dloss_dsdf}), by Theorem~\ref{theo}, we obtain $\frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \mathbf{e}} = 0$ and $\frac{\partial \frac{\partial \mathbf{e}}{\partial \mathbf{x}}}{\partial \Theta} = 0$. 
%
This results in the following simplified form
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:simplified_dloss_denc}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \Omega}
&= \frac{\partial \mathcal{L}}{\partial \mathbf{n}} \frac{\partial d}{\partial \mathbf{e}} \frac{\partial \frac{\partial \mathbf{e}}{\partial \mathbf{x}}}{\partial \Omega}
\end{aligned}
\end{equation}

\begin{equation} \label{eqn:simplified_dloss_dmlp}
\begin{aligned}
\frac{\partial \mathcal{L}}{\partial \Theta} (n)
&= 
\frac{\partial \mathcal{L}}{\partial \mathbf{n}} 
\frac{\partial \mathbf{e}}{\partial \mathbf{x}} \frac{\partial \frac{\partial d}{\partial \mathbf{e}}}{\partial \Theta} 
% \\&= \frac{\partial \mathcal{L}}{\partial n} \frac{\partial enc}{\partial x} \frac{\partial \frac{\partial sdf}{\partial enc}}{\partial \theta_\mathrm{sdf}} 
\end{aligned}
\end{equation}
%%%%%%%%%%%%
%
for the second-order derivatives resulting in improved efficiency and less computational overhead.
%
%%%%%%%%%%%%
%
\subsection{Progressive Training} \label{sec:progessive}
%
Although our highly-optimized gradient calculation already improved training time, we found there is still room for improvement in terms of training convergence.
%
We empirically observed that using grids at low resolutions results in underfitting of the data, in which the geometry reconstruction is smooth and lacks details, whereas using grids at high resolutions induces over-fitting, leading to increased noise and artifacts of the results.
%
Therefore, we introduce a progressive training method by gradually increasing the bandwidth of our spatial grid encoding denoted as:
%
%%%%%%%%%%%%
\begin{equation}
   h_\Omega(\mathbf{x}, \lambda) = \big(w_1(\lambda) h_\Omega^1(\mathbf{x}), \dots, w_{L}(\lambda)  h_\Omega^L(\mathbf{x}) \big), 
\end{equation}
%%%%%%%%%%%%
%
where $h_\Omega^i$ is the hash encoding at level $i$ and the weight $w_i$ for each grid encoding level is defined by
%
%%%%%%%%%%%%
\begin{equation}
w_i(\lambda)=
\begin{cases}
0, \text{ if } i>\lambda \\
1, \text{ otherwise} 
\end{cases},
\end{equation}
%%%%%%%%%%%%
%
and the parameter $\lambda$ modulates the bandwidth of the low-pass filter applied to the multi-resolution hash encodings, which gradually increases during the training process.
%
\MH{the notation introduced above is not consistent with the previous notations. there has to be a link to the hashgrid $h_\Omega$ notation and maybe $\mathbf{e}$, otherwise it is not clear where this step is applied and how it links to previous things we introduced. \yiming{finished}}
%
The intuition here is that we learn the scene geometry in a coarse-to-fine manner, and our results demonstrate that convergence time can be significantly improved by this design choice.
%
More details are provided in the supplemental document.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
\section{Dynamic Neural Surface Reconstruction} \label{sec:method_dynamic}
%
So far, we explained how NeuS2 can obtain highly accurate and fast reconstructions of static scenes. 
%
Next, we extend NeuS2 to dynamic scene reconstruction. 
%
That is, given multi-view videos of a moving object and camera parameters of each view, our goal is to learn the neural implicit surfaces of the object in each video frame (see Fig.~\ref{fig:overview} b)). 
%
%%%%%%%%%%%%
%
\subsection{Incremental Training} \label{sec:incremental}
%
Even though our reconstruction method of static objects can achieve promising efficiency and quality, constructing dynamic scenes by training every single frame independently is still time-consuming.
%
However, scene changes from one frame to the other are typically small.
%
Thus, we propose an incremental training strategy to exploit the similarity in geometry and appearance information shared between two consecutive frames, which enables faster convergence of our model.
%
In detail, we train the first frame from scratch as illustrated in our static scene reconstruction, and then fine-tune the model parameters for the subsequent frames based on the learned representation of the previous frame.
%
Using this strategy, the model is able to establish a feasible initialization of the neural representation of the target frame and, thus, significantly accelerates its convergence speed.
%
%%%%%%%%%%%%
%
\subsection{Global Transformation Prediction} \label{sec:transform}
%
\MH{not nicely explained --> see skype chat! we should motivate this better \yiming{finished. Add one paragraph mentioned in skype}}
%
As we observed during the incremental training process, for some regions that are occluded in most camera views, the predicted SDF may get stuck in the learned SDF of the previous frame as the local minima, when the object's movement between adjacent frames is relatively large.
%
For instance, when our model reconstructs a walking sequence from muli-view images, the reconstructed surface appears to have many holes, as shown in figure \ref{fig:ablation_dynamic}. \LJ{show a figure as an example \yiming{refer to the ablation study}}.
%
To address this issue, we propose a global transformation prediction to roughly transform the target SDF into a canonical space before the incremental training.
%
Specifically, we predict the rotation $R$ and transition $T$ of the object between two adjacent frames. 
%
For any given 3D position $\mathbf{x}_i$ in the coordinate space of the frame $i$, it is transformed back to the coordinate space of the previous frame $i-1$, defined as $\mathbf{x}_{i-1}$
%
%%%%%%%%%%%%
\begin{equation} \label{eqn:globalmove_predict}
    \mathbf{x}_{i-1}=R_i(\mathbf{x}_{i}+T_i).
\end{equation}
%%%%%%%%%%%%
%
The transformations can then be accumulated to transform the point $\mathbf{x}_i$ back to $\mathbf{x}_c$ in the first frame's coordinate space
%
%%%%%%%%%%%%
\begin{equation}
    \mathbf{x}_c=R_{i-1}^c(\mathbf{x}_{i-1}+T_{i-1}^c)=R_{i}^c(\mathbf{x}_{i}+T_{i}^c),
\end{equation}
%%%%%%%%%%%%
%
where $R_i^c=R_{i-1}^cR_i$ and $T_i^c=T_i+R_i^{-1}T_{i-1}^c$.
%
%%%%%%%%%%%%
%
\par
%
% \yiming{Another benefit of the global transformation prediction is that we can model the dynamic scenes with large movement in a small region, instead of using a very large hash grid to cover the entire scene. Since the hash grid only need to model a small portion of the entire scene, we can get more accurate reconstruction and reduce the memory costs.}
% \yiming{Note that another benefit of the global transformation prediction is that we can build our hash grid only in a small region, instead of enlarging the hash grid to cover the entire scene.}
The Global Transformation Prediction also allows us to model dynamic sequences with large movement in a small region, rather than covering the entire scene with a large hash grid. 
Since the hash grid only needs to model a small portion of the entire scene, we can obtain more accurate reconstructions and reduce memory costs.

% %
% %%%%%%%%%%%%
% %
% \par
% %
% By 
% Note that this transformation definition in Eq.~\ref{eqn:globalmove_predict} explicitly separates the rotation from transition, compared with the alternative form $X_{i-1}=R_iX_{i}+T_i$ \LJ{more derivations are needed, may be included in the supply.}, which enables better learning efficiency and accuracy. 
%
%%%%%%%%%%%%
%
\par
%
Notably, our method can handle large movements which are challenging for existing dynamic scene reconstruction approaches\cite{tretschk2020nonrigid}, \cite{park2020nerfies}, thanks to the designs of our approach: 
%
(1) Global transformation prediction that accounts for large global  movements in the sequence; 
%
(2) Incremental training that learns relatively small deformable movements between two adjacent frames rather than learns relatively large movements from each frame to a common canonical space.  
%
%%%%%%%%%%%%
%
\par
%
We achieve our incremental training combined with global transformation prediction as an end-to-end learning scheme, as illustrated in figure~\ref{fig:overview}(b).
%
When turning to a new frame, we first predict the global transformation independently, and upon training convergence for the global prediction, we fine-tune the model's parameters and global transformation together to efficiently learn the neural representation.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We implement the second-order derivative of ReLU based MLP in CUDA for the SDF network and use the second-order derivative implementation in \textit{tiny-cuda-nn} for the hash grid. 
% \textbf{Theorem 1} (The second-order derivative of the MLP) \label{second_order_derivative}
% Given a \textit{ReLU} based MLP $f$ with $L$ hidden layers taking $x \in \mathbb{R}^{d}$ as input, it layer-wisely computes $x_l = R(H_lx_{l-1})$, where $l\in \{1,\dots,L\}$ is the layer index, $x_0 = x$, $ x_l \in \mathbb{R}^{n_l}$, $H_l \in \mathbb{R}^{n_l \times n_{l-1}}$ and $R$ is the ReLU function. The second-order derivative formula of the MLP $f$ is:
% \begin{equation}
% \frac{\partial \frac{\partial y}{\partial x}}{\partial H_l} = (H_{l+1}^T \dots RH_L^TS_L) (H_{l-1} \dots RH_1S_1)
% % d(dy\_dx)\_d(H^i_{mn}) = 
% % \Sigma_k \{H^1 R H^2 \dots R H^{i-1} R\}_{kn} * \Sigma_l \{RH^{i+1} \dots RH^n\}_{ml}
% \end{equation}
% \begin{equation}
% \frac{\partial^2 y}{\partial \mathbf{x}^2} = 0
% \end{equation}


% We implement the second-order derivative of ReLU based MLPs in CUDA for the SDF network and use the second-order derivative implementation in \textit{tiny-cuda-nn} for the hash grid. 
% Given the loss function $\mathcal{L}$, we optimize the parameters hash grids calculate the second-order gradient of the hash grids $\vect{F_{hash}}$ and the SDF network $f_\mathrm{sdf}$ based on the chain rule of derivatives.

% \textbf{Lemma 1} (Chain rules for second-order derivative) \label{second_order_derivative}
% Suppose two networks $f_1(\mathbf{\theta_1}), f_2(\mathbf{\theta_2})$, where $\theta_1$ and $\theta_2 $ are the network's learnable parameters, are combined to form a mapping $f = f_2 \cdot f_1 $. Given an input $ \mathbf{x}$, the network computes $f(\mathbf{x}) = f_2( f_1(\mathbf{x}))$. We denote $ y_1 = f_1(x)$ and $y_2 = f_2(y_1)$. For a loss function $L$ that is relevant to the gradient term $\nabla_{\mathrm{\mathbf{x}}}{f}$, e.g. the Eikonal loss $\left(\left\|\nabla_{\mathrm{\mathbf{x}}}{f} \right\|_2-1\right)^2 $, the second-order derivatives according to $\mathbf{x}, \mathbf{\theta_1}, \mathbf{\theta_2}$ are:


% \begin{equation}
% \frac{\partial^2 L}{\partial \mathbf{x}^2} =
% \end{equation}

% \begin{equation}
% \frac{\partial^2 L}{\partial \mathbf{\theta_1}^2} =
% \end{equation}

% \begin{equation}
% \frac{\partial^2 L}{\partial \mathbf{\theta_2}^2} =
% \end{equation}

==> x_preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% common preambles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{graphicx}
% DO NOT USE \usepackage{times}, it will be removed by typesetters
%\usepackage{times}

\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{color}
\usepackage{ulem}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

%--------------------------------------------------
% colored text and comments
%--------------------------------------------------
\usepackage{bm}
% \newcommand{\blue}[1]{\textcolor{blue}{{#1}}}
% \newcommand{\LJ}[1]{{\textcolor{blue}{[\textbf{LJ:]} #1}}}
% \newcommand{\MH}[1]{\textcolor{cyan}{[\textbf{Marc:}]:#1}}
% \newcommand{\hanqin}[1]{\textcolor{red}{[hanqin]:#1}}
% \newcommand{\yiming}[1]{\textcolor{red}{[yiming]:#1}}
% \newcommand{\remove}[1]{\textcolor{blue}{{[To remove]:#1}}}
% \newcommand{\change}[1]{{\textcolor{cyan}{#1}}}


%--------------------------------------------------
% for vectors (should be surrounded by $)
%--------------------------------------------------
%\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{multirow}
%\usepackage{mathtools}
\usepackage{mathrsfs}
\newcommand{\isep}{\mathrel{{.}\,{.}}\nobreak}
\newcommand{\vect}[1]{{\bm{#1}}}
\newcommand{\unit}[1]{\widehat{#1}}
\newcommand{\sign}[1]{\operatorname{sign}(#1)}
\newcommand{\vecangle}[2]{(#1,#2)}

%--------------------------------------------------
% common shortcuts in the text
%--------------------------------------------------
\usepackage{xspace}
% \newcommand{\ie}{\textsl{i.e.}~}
% \newcommand{\eg}{\textsl{e.g.}~}
% \newcommand{\etal}{\textsl{et~al.}~}
% \newcommand{\wrt}{\textsl{w.r.t.}~}
\newcommand{\NB}{\textsl{NB:}~}
% \newcommand{\vs}{\textsl{vs.}~}
% \newcommand{\cf}{\textsl{cf.}~}
\newcommand{\resp}{respectively\xspace}
\newcommand{\aka}{\textsl{a.k.a.}~}

%--------------------------------------------------
% Commands for keeping text (it's in the latex
%  but not displayed on pdf)
%--------------------------------------------------
\newcommand{\keep}[1]{}
\newcommand{\old}[1]{}

%--------------------------------------------------
% Math operators
%--------------------------------------------------
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\softmax}{softmax}
\DeclareMathOperator*{\GCN}{GCN}
\DeclareMathOperator*{\CNN}{CNN}
\DeclareMathOperator*{\MLP}{MLP}
\DeclareMathOperator*{\DeGCN}{GCN*}
\DeclareMathOperator*{\FwdSkin}{SMPL}
\DeclareMathOperator*{\BwdSkin}{\mathcal{G}}


% Recommended, but optional, packages for figures and better typesetting:
\usepackage{times}
\usepackage{epsfig}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% \usepackage{subfig}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2021} with \usepackage[nohyperref]{icml2021} above.
\usepackage{hyperref}
% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}} 
\newcommand{\eqnref}[1]{{Equation~{#1}}}
\newcommand{\figref}[1]{{Figure~{#1}}}
